Weight Vector Tuning and Asymptotic Analysis of Binary Linear Classifiers

Unlike its intercept, a linear classifier's weight vector cannot be tuned by a simple grid search. Hence, this paper proposes weight vector tuning of a generic binary linear classifier through the parameterization of a decomposition of the discriminant by a scalar which controls the trade-off between conflicting informative and noisy terms. By varying this parameter, the original weight vector is modified in a meaningful way. Applying this method to a number of linear classifiers under a variety of data dimensionality and sample size settings reveals that the classification performance loss due to non-optimal native hyperparameters can be compensated for by weight vector tuning. This yields computational savings as the proposed tuning method reduces to tuning a scalar compared to tuning the native hyperparameter, which may involve repeated weight vector generation along with its burden of optimization, dimensionality reduction, etc., depending on the classifier. It is also found that weight vector tuning significantly improves the performance of Linear Discriminant Analysis (LDA) under high estimation noise. Proceeding from this second finding, an asymptotic study of the misclassification probability of the parameterized LDA classifier in the growth regime where the data dimensionality and sample size are comparable is conducted. Using random matrix theory, the misclassification probability is shown to converge to a quantity that is a function of the true statistics of the data. Additionally, an estimator of the misclassification probability is derived. Finally, computationally efficient tuning of the parameter using this estimator is demonstrated on real data.

==> citations.tex <==
@article{mai2012direct,
  title={A direct approach to sparse discriminant analysis in ultra-high dimensions},
  author={Mai, Qing and Zou, Hui and Yuan, Ming},
  journal={Biometrika},
  volume={99},
  number={1},
  pages={29--42},
  year={2012},
  publisher={Oxford University Press}
}

%phoneme dataset from https://web.stanford.edu/~hastie/ElemStatLearn/datasets/phoneme.info.txt
@article{hastie1995penalized,
  title={Penalized discriminant analysis},
  author={Hastie, Trevor and Buja, Andreas and Tibshirani, Robert},
  journal={The Annals of Statistics},
  pages={73--102},
  year={1995},
  publisher={JSTOR}
}

@inproceedings{hachem2013bilinear,
  title={On bilinear forms based on the resolvent of large random matrices},
  author={Hachem, Walid and Loubaton, Philippe and Najim, Jamal and Vallet, Pascal},
  booktitle={Annales de l'IHP Probabilit{\'e}s et statistiques},
  volume={49},
  number={1},
  pages={36--63},
  year={2013}
}

@article{kammoun2019asymptotic,
  title={Asymptotic analysis of RZF in large-scale {MU-MIMO} systems over Rician channels},
  author={Kammoun, Abla and Sanguinetti, Luca and Debbah, Merouane and Alouini, Mohamed-Slim},
  journal={IEEE Transactions on Information Theory},
  volume={65},
  number={11},
  pages={7268--7286},
  year={2019},
  publisher={IEEE}
}

@article{muller2016random,
  title={Random matrix theory tutorial-{I}ntroduction to deterministic equivalents},
  author={Muller, Axel and Debbah, M{\'e}rouane},
  journal={Traitement du signal},
  volume={33},
  number={2-3},
  pages={223--248},
  year={2016},
  publisher={PRESSES UNIV GRENOBLE 1041 RUE DES RESIDENCES, GRENOBLE, 38040, FRANCE}
}

@article{weisstein2017hypersphere,
  title={Hypersphere {P}oint {P}icking},
  author={Weisstein, Eric W},
  journal={From MathWorld--A Wolfram Web Resource},
  note={Available at http://mathworld.wolfram.com/HyperspherePointPicking.html},
  year={2017}
}

@inproceedings{durrant2013random,
  title={Random projections as regularizers: Learning a linear discriminant ensemble from fewer observations than dimensions},
  author={Durrant, Robert J. and Kab{\'a}n, Ata},
  year={2013},
  publisher={JMLR},
  pages = {17--32},
  volume={29},
  booktitle = {Proceedings of the Asian Conference on Machine Learning},
  url = {http://jmlr.org/proceedings/papers/v29/Durrant13.html Google Scholar}
}


@article{yuan2012recent,
  title={Recent advances of large-scale linear classification},
  author={Yuan, Guo-Xun and Ho, Chia-Hua and Lin, Chih-Jen},
  journal={Proceedings of the IEEE},
  volume={100},
  number={9},
  pages={2584--2603},
  year={2012},
  publisher={IEEE}
}

@article{friedman1989regularized,
  title={Regularized discriminant analysis},
  author={Friedman, Jerome H},
  journal={Journal of the American statistical association},
  volume={84},
  number={405},
  pages={165--175},
  year={1989},
  publisher={Taylor \& Francis}
}

@article{di1976application,
  title={The application of bias to discriminant analysis},
  author={Di Pillo, Pasquale J},
  journal={Communications in Statistics-Theory and Methods},
  volume={5},
  number={9},
  pages={843--854},
  year={1976},
  publisher={Taylor \& Francis}
}

@article{guo2007regularized,
  title={Regularized linear discriminant analysis and its application in microarrays},
  author={Guo, Yaqian and Hastie, Trevor and Tibshirani, Robert},
  journal={Biostatistics},
  volume={8},
  number={1},
  pages={86--100},
  year={2007},
  publisher={Oxford University Press}
  }
  
  @inproceedings{le1990handwritten,
  title={Handwritten zip code recognition with multilayer networks},
  author={Le Cun, Yann and Matan, Ofer and Boser, Bernhard and Denker, John S and Henderson, Don and Howard, Richard E and Hubbard, Wayne and Jacket, LD and Baird, Henry S},
  booktitle={[1990] Proceedings. 10th International Conference on Pattern Recognition},
  volume={2},
  pages={35--40},
  year={1990},
  organization={IEEE}
}

@inproceedings{fradkin2008clustering,
  title={Clustering inside classes improves performance of linear classifiers},
  author={Fradkin, Dmitriy},
  booktitle={2008 20th IEEE International Conference on Tools with Artificial Intelligence},
  volume={2},
  pages={439--442},
  year={2008},
  organization={IEEE}
}

@article{duda2001pattern,
  title={Pattern classification},
  author={Duda, Richard O and Stork, David G and Hart, Peter E},
  year={2001},
  publisher={Wiley}
}

@incollection{MARQUAND202083,
title = "Chapter 5 - Linear methods for classification",
editor = "Andrea Mechelli and Sandra Vieira",
booktitle = "Machine Learning",
publisher = "Academic Press",
pages = "83 - 100",
year = "2020",
isbn = "978-0-12-815739-8",
doi = "https://doi.org/10.1016/B978-0-12-815739-8.00005-5",
url = "http://www.sciencedirect.com/science/article/pii/B9780128157398000055",
author = "Andre F. Marquand and Seyed Mostafa Kia",
keywords = "Autism spectrum disorder, Automated diagnosis, Bayesian models, Brain decoding, Brain disorders, Clinical neuroimaging, Linear classification models, Penalized linear models, Schizophrenia, Sparsity, Structured sparsity",
abstract = "Linear classification methods are highly prevalent in clinical neuroimaging and have been used to predict diagnosis and outcome in many brain disorders. Here, we provide a concise introduction to these methods aimed at the beginning practitioner. We introduce the two main variants: penalized linear models and probabilistic classification models, highlighting their relative strengths and weaknesses. We describe discriminative mapping, which is the ability to visualize the model coefficients in the input space and is a crucial benefit of linear models because it helps to understand which features of the data drive the predictions. We also introduce the notion of sparsity, which further assists interpretation in that it can be used to restrict the discriminative pattern to a small number of brain regions. Finally, we provide an overview of studies using linear models along with two illustrative applications using linear models to discriminate patients with autism and schizophrenia from healthy participants."
}

@article{wen2020performance,
  title={Performance of linear classification algorithms on $\alpha$/$\gamma$ discrimination for LaBr3: Ce scintillation detectors with various pulse digitizer properties},
  author={Wen, Jingjun and Zhu, Jinfu and Xue, Tao and Cang, Jirong and Wei, Liangjun and Nie, Qiyuan and Zeng, Ming and Zeng, Zhi and Ma, Hao and Li, Jianmin and others},
  journal={Journal of Instrumentation},
  volume={15},
  number={02},
  pages={P02004},
  year={2020},
  publisher={IOP Publishing}
}

@article{berry2019linear,
  title={Linear classification scores in beef cattle as predictors of genetic merit for individual carcass primal cut yields},
  author={Berry, Donagh P and Pabiou, Thierry and Fanning, Rory and Evans, Ross D and Judge, Michelle M},
  journal={Journal of animal science},
  volume={97},
  number={6},
  pages={2329--2341},
  year={2019},
  publisher={Oxford University Press US}
}

@article{randhawa2020machine,
  title={Machine learning using intrinsic genomic signatures for rapid classification of novel pathogens: {COVID}-19 case study},
  author={Randhawa, Gurjit S and Soltysiak, Maximillian PM and El Roz, Hadi and de Souza, Camila PE and Hill, Kathleen A and Kari, Lila},
  journal={Plos one},
  volume={15},
  number={4},
  pages={e0232391},
  year={2020},
  publisher={Public Library of Science San Francisco, CA USA}
}

@inproceedings{ashok2019strategy,
  title={Strategy representation by decision trees with linear classifiers},
  author={Ashok, Pranav and Br{\'a}zdil, Tom{\'a}{\v{s}} and Chatterjee, Krishnendu and K{\v{r}}et{\'\i}nsk{\`y}, Jan and Lampert, Christoph H and Toman, Viktor},
  booktitle={International Conference on Quantitative Evaluation of Systems},
  pages={109--128},
  year={2019},
  organization={Springer}
}

@article{alanni2019novel,
  title={A novel gene selection algorithm for cancer classification using microarray datasets},
  author={Alanni, Russul and Hou, Jingyu and Azzawi, Hasseeb and Xiang, Yong},
  journal={BMC medical genomics},
  volume={12},
  number={1},
  pages={10},
  year={2019},
  publisher={Springer}
}

@article{zollanvari2019asymptotically,
  title={Asymptotically Bias-Corrected Regularized Linear Discriminant Analysis for Cost-Sensitive Binary Classification},
  author={Zollanvari, Amin and Abdirash, Muratkhan and Dadlani, Aresh and Abibullaev, Berdakh},
  journal={IEEE Signal Processing Letters},
  volume={26},
  number={9},
  pages={1300--1304},
  year={2019},
  publisher={IEEE}
}

@article{wang2018dimension,
  title={On the dimension effect of regularized linear discriminant analysis},
  author={Wang, Cheng and Jiang, Binyan and others},
  journal={Electronic Journal of Statistics},
  volume={12},
  number={2},
  pages={2709--2742},
  year={2018},
  publisher={The Institute of Mathematical Statistics and the Bernoulli Society}
}

@article{benaych2016spectral,
  title={Spectral analysis of the Gram matrix of mixture models},
  author={Benaych-Georges, Florent and Couillet, Romain},
  journal={ESAIM: Probability and Statistics},
  volume={20},
  pages={217--237},
  year={2016},
  publisher={EDP Sciences}
}

@book{couillet2011random,
  title={Random matrix methods for wireless communications},
  author={Couillet, Romain and Debbah, Merouane},
  year={2011},
  publisher={Cambridge University Press}
}

@MISC {875205,
    TITLE = {Uniformly bounded derivative implies uniform convergence},
    AUTHOR = {Daniel Fischer (https://math.stackexchange.com/users/83702/daniel-fischer)},
    HOWPUBLISHED = {Mathematics Stack Exchange},
    NOTE = {URL:https://math.stackexchange.com/q/875205 (version: 2014-07-22)},
    EPRINT = {https://math.stackexchange.com/q/875205},
    URL = {https://math.stackexchange.com/q/875205}
}

@book{friedman2001elements,
  title={The elements of statistical learning},
  author={Friedman, Jerome and Hastie, Trevor and Tibshirani, Robert},
  volume={1},
  number={10},
  year={2001},
  publisher={Springer series in statistics New York}
}

@incollection{bai2008limit,
  title={Limit of the smallest eigenvalue of a large dimensional sample covariance matrix},
  author={Bai, Zhi-Dong and Yin, Yong-Qua},
  booktitle={Advances In Statistics},
  pages={108--127},
  year={2008},
  publisher={World Scientific}
}

@article{kammoun2014smallest,
  title={On the Smallest Eigenvalue of General correlated Gaussian Matrices},
  author={Kammoun, Abla and Alouini, Mohamed-Slim},
  journal={arXiv preprint arXiv:1412.8340},
  year={2014}
}

@article{sifaou2020high,
  title={High-dimensional Linear Discriminant Analysis Classifier for Spiked Covariance Model},
  author={Sifaou, Houssem and Kammoun, Abla and Alouini, Mohamed-Slim},
  journal={Journal of Machine Learning Research},
  volume={21},
  pages={1--24},
  year={2020}
}


@article{huang2010bias,
  title={Bias-corrected diagonal discriminant rules for high-dimensional classification},
  author={Huang, Song and Tong, Tiejun and Zhao, Hongyu},
  journal={Biometrics},
  volume={66},
  number={4},
  pages={1096--1106},
  year={2010},
  publisher={Wiley Online Library}
}

@ONLINE {niyazi2020asymptoticARXIV,
    author = "Lama B. Niyazi and Abla Kammoun and Hayssam Dahrouj and Mohamed-Slim Alouini and Tareq Y. Al-Naffouri",
    title  = "Asymptotic Analysis of an Ensemble of Randomly Projected Linear Discriminants",
    year   = "2020",
    url    = "https://arxiv.org/abs/2004.08217"
}

@article{niyazi2020asymptotic,
  title={Asymptotic Analysis of an Ensemble of Randomly Projected Linear Discriminants},
  author={Niyazi, Lama B and Kammoun, Abla and Dahrouj, Hayssam and Alouini, Mohamed-Slim and Al-Naffouri, Tareq Y},
  journal={IEEE Journal on Selected Areas in Information Theory},
  volume={1},
  number={3},
  pages={914--930},
  year={2020},
  publisher={IEEE}
}
